Tune it the Right Way: Unsupervised Validation of Domain Adaptation via Soft Neighborhood Density

Unsupervised domain adaptation (UDA) methods can dramatically improve generalization on unlabeled target domains. However, optimal hyper-parameter selection is critical to achieving high accuracy and avoiding negative transfer. Supervised hyper-parameter validation is not possible without labeled target data, which raises the question: How can we validate unsupervised adaptation techniques in a realistic way? We first empirically analyze existing criteria and demonstrate that they are not very effective for tuning hyper-parameters. Intuitively, a well-trained source classifier should embed target samples of the same class nearby, forming dense neighborhoods in feature space. Based on this assumption, we propose a novel unsupervised validation criterion that measures the density of soft neighborhoods by computing the entropy of the similarity distribution between points. Our criterion is simpler than competing validation methods, yet more effective; it can tune hyper-parameters and the number of training iterations in both image classification and semantic segmentation models. The code used for the paper will be available at \url{https://github.com/VisionLearningGroup/SND}.

==> latex/figures/main_figure.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{latex/images/method.jpg}
    \caption{{\bf Method overview.} \ours measure the density of clustered target features using unlabeled target samples, which is used to select hyper-parameters including checkpoints.}
    \label{fig:overview}
\end{figure*}

==> latex/figures/oh_p2c_partial_nc.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{latex/images/oh_p2c_partial_nc.jpg}
    \caption{Product to Clipart (OfficeHome) adaptation results in partial DA. NC~\cite{saito2020universal} is used as an adaptation method.}
    \label{fig:overview}
\end{figure*}

==> latex/figures/toy_data.tex <==
\begin{figure}[!t]
{\small
\begin{center}
 \begin{subfigure}[Source]{0.49\hsize}
  \begin{center}
   \includegraphics[width=\hsize, height=0.8\hsize]{latex/images/var_0.5.jpg}
    \caption{Var = 0.5, SIE = 5.704.}
  \end{center}
 \end{subfigure}
 \begin{subfigure}[Target]{0.49\hsize}
  \begin{center}
   \includegraphics[width=\hsize, height=0.8\hsize]{latex/images/var_2.5.jpg}
    \caption{Var = 2.5, SIE = 5.657.}
  \end{center}
 \end{subfigure}
 \vspace{-5mm}
  \caption{Toy data experiments to see the relationship between the variance within the same class and similarity entropy. Red and green plots show different classes. The black line is the learnt decision boundary. As shown in these results, the value of similarity entropy is larger if the variance is smaller.}
   \label{fig:toy}
   \end{center}
}
\end{figure}


==> latex/figures/toy_distance_source.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{latex/images/toy_distance_source.png}
    \caption{\oursv with respect to the distance between source and target. Left: \oursv. Right: Accuarcy.}
    \label{fig:toy_distace_source}
\end{figure}

==> latex/figures/toy_margin.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{latex/images/toy_margin.png}
    \caption{\oursv with respect to between-class distance. Left: \oursv. Right: Accuarcy.}
    \label{fig:toy_distace}
\end{figure}

==> latex/figures/toy_num_classes.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{latex/images/num_classes.jpg}
    \vspace{-7mm}
    \caption{\oursv with respect to the number of classes. Left (a)(b): Plots of varying the number of classes. We vary the number of classes while fixing the number of samples used to compute \oursv. In this way, we observe the behavior of \oursv by changing the number of classes. Right: The change of \oursv and accuracy with respect to the number. Since the concentration degree decreases with the increase of the number of classes, \oursv gets smaller with the increase.}
    \label{fig:toy_classes}
\end{figure*}

==> latex/tables/main_table.tex <==
\begin{table*}[t]
\scalebox{1.0}{
\begin{tabular}{l||c||cccccccc|c}
Methods                          & Labeled & CUB          & Flower       & Caltech & Clipart & Art    & Satellite & Texture & iNat  & Avg      \\\hline
Rotation & N&0.218&&&&&0.525&& \\
Entropy                                             & Y               & 0.109        &              &         & 0.294   & 0.388  &               &         &             \\
%Imagenet Entropy                 & Y                   & N               & 0.180        & 0.093        & 0.455   & 0.573   &        & 0.055         & 0.437   & 0.509       \\
Ours / Kmeans Acc                            & N               & 0.748        & 0.851        & 0.917        & 0.719   & 0.762  & 0.375         & 0.556   &       0.609      \\
%Ours / ImageNet Softmax          & Y                   & N               & 0.810        & 0.391        & 0.947   & 0.700   & 0.923  & 0.112         & 0.261   & 0.635       \\
Ours / Sim-Entropy                    & Y               & 0.799        & 0.970        & 0.965   & 0.850   & 0.757  & 0.718         & 0.805   & 0.558  \\\hline
\end{tabular}}
\caption{Results in transfer learning.}
\end{table*}


==> latex/tables/nc_all.tex <==
\begin{table*}[]
\begin{tabular}{l|cccc|ccc|cccc}
	\toprule[1.0pt]
	\multirow{2}{*}{Method}  &  \multicolumn{4}{c|}{Closed DA} &\multicolumn{3}{c|}{Partial DA}  &\multicolumn{4}{c|}{Open set DA}     \\
 & A2D & W2A & R2A& A2P & R2A & A2P & P2C & A2D &W2A &R2A &A2P\\\hline
Lower Bound\\\hline 
Source Risk \\
DEV~\cite{you2019towards}\\
Entropy~\cite{morerio2017minimal}&87.9&66.2\\
Ours &87.9&66.2\\ \hline 
Upper Bound (Target Risk) \\ 
	\bottomrule[1.0pt]
\end{tabular}
\caption{Adapted by NC~\cite{saito2020universal}.}
\end{table*}


==> latex/tables/validation_prior_work.tex <==
\begin{table}[]
\begin{center}
    
\begin{tabular}{l|c}
	\toprule[1.0pt]
	
Method  & List of papers\\\hline
\bf{Source Risk} &\cite{ganin2014unsupervised,sun2015return,cao2018partial}\\
\bf{Target Risk}&\cite{shrivastava2017learning,bousmalis2017unsupervised,bousmalis2016domain,ghifary2016deep,saito2017asymmetric,shu2018dirt,russo2018source}\\
\bf{Fixed parameters}&\cite{tzeng2017adversarial,long2016unsupervised,saito2017maximum,sankaranarayanan2018generate}\\
%\bf{Entropy}&\cite{morerio2017minimal}\\
\bf{IWV}~\cite{sugiyama2007covariate, you2019towards}&\cite{long2017conditional,cao2018partial,jin2020minimum,wang2019transferable,you2019towards}\\
\bf{Not mentioned}&\cite{cycada,tzeng2015simultaneous,sun2016deep,tsai2018learning,murez2018image,zou2018unsupervised,zhang2018collaborative,volpi2018adversarial,vu2018advent}\\
	\bottomrule[1.0pt]
\end{tabular}
\end{center}
\vspace{-7mm}
\caption{{\small List of validation methods for unsupervised domain adaptation used by prior works.}}
\label{tb:prior_validation}

\end{table}

